Modeling the fast optical transient SN 2019bkc/ATLAS19dqr with a central engine and implication for its origin

Modern wide-field high-cadence surveys have revealed the significant diversity of optical transient phenomena in their luminosity and timescale distributions, which led to the discovery of some mysterious fast optical transients (FOTs). These FOTs can usually rise and decline remarkably in a timescale of a few days to weeks, which are obviously much rapider than ordinary supernovae. SN 2019bkc/ATLAS19dqr is one of the fastest detected FOTs so far and, meanwhile, it was found to be un-associated with a host galaxy. These discoveries provide a good chance to explore the possible origins of FOTs. So, we model the light curves of SN 2019bkc in details. It is found that SN 2019bkc can be well explained by the thermal emission of an explosion ejecta that is powered by a long-lasting central engine. The engine could be a spinning-down millisecond magnetar or a fallback accretion onto a compact object. Combining the engine property, the mass of the ejecta, and the hostlessness of SN 2019bkc, we suggest that this FOT is likely to originate from a merger of a white dwarf and a neutron star.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

